ROOT: Requirements Organization and Optimization Tool

Software engineering practices such as constructing requirements and establishing traceability help ensure systems are safe, reliable, and maintainable. However, they can be resource-intensive and are frequently underutilized. To alleviate the burden of these essential processes, we developed the Requirements Organization and Optimization Tool (ROOT). ROOT centralizes project information and offers project visualizations and AI-based tools designed to streamline engineering processes. With ROOT's assistance, engineers benefit from improved oversight and early error detection, leading to the successful development of software systems. Link to screen cast: https://youtu.be/3rtMYRnsu24

==> format.tex <==
\usepackage[T1]{fontenc}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{xcolor}
\usepackage{url}
\usepackage{array}
\usepackage{color}
\usepackage{wasysym}
\usepackage{verbatim}
\usepackage{bigstrut}
\usepackage{multirow}
\usepackage{setspace}
\usepackage{tabularx}
\usepackage{xspace}
\usepackage{subcaption}
\usepackage[font=footnotesize]{caption}
\usepackage{soul}
\usepackage{vcell}
\usepackage{pifont}
\usepackage{afterpage}
\usepackage{rotating}

\usepackage{graphicx}
\usepackage{enumitem}

\usepackage{balance}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{algpseudocode}
\usepackage{hyperref}
\usepackage{ulem}
\usepackage{amssymb}
\usepackage{wrapfig}
\usepackage{tcolorbox}

\newcommand{\jch}[1]{{\textcolor{blue}{#1}}} %blue
\newcommand{\kd}[1]{{\textcolor{red}{#1}}} %red

\definecolor{dkgreen}{HTML}{006400}
\newcommand{\ar}[1]{\textcolor{dkgreen}{#1}} %green

==> tables/coverage.tex <==
% \begin{table}[t]
%   \centering
%   \caption{Percentage of Concepts from Original Documentation Captured Per HGEN Version.}
%   \label{tab:coverage}
%   \begin{tabular}{c|ccc}
%   \hline
%   \textbf{Project} & \textbf{Method} & \textbf{\% Covered} & \textbf{\% Used} \\ \hline \hline
%   \multirow{2}{*}{Dronology} & Baseline & 6.3\% & 9.1\% \\
%    & HGEN  & 87.5\%  & 28.9\% \\ \hline
%   \multirow{2}{*}{SAFA}  & Baseline  & 37.8\%  & 38.9\% \\
%    & HGEN  & 84.4\%  & 43.1\% \\ \hline
%   \multirow{2}{*}{JOC} & Baseline  & 50.0\%  & 35.7\% \\
%    & HGEN  & 100\%  & 38.5\% \\ \hline
%   \end{tabular}
% \end{table}

\begin{table}[t]
  \centering
  \caption{Percentage of Concepts from Original Documentation Captured Per HGEN Version, as determined by the Project Experts (E1-E3).}
  \label{tab:coverage}
    \addtolength{\tabcolsep}{-3.5pt}
  \begin{tabular}{c|c|cc|cc}
  \hline
  \multirow{2}{*}{\textbf{Project}} &\multirow{2}{*}{\textbf{ID}}& \multicolumn{2}{c|}{\textbf{Baseline}} & \multicolumn{2}{c}{\textbf{HGEN}} \\ \cline{3-6} 
   && \textbf{\% Covered} & \textbf{Covered by} & \textbf{\% Covered} & \textbf{Covered by} \\ \hline \hline
  Dronology & E1& 6.3\% & 9.1\% & 87.5\% & 28.9\% \\ \hline
  SAFA & E2 & 37.8\% & 38.9\% & 84.4\% & 43.1\% \\ \hline
  JOC & E3& 50.0\% & 35.7\% & 100\% & 38.5\% \\ \hline
  \end{tabular}
  \vspace{-12pt}
\end{table}



==> tables/coverage_examples.tex <==
\begin{table}
\centering
\caption{Examples of HGEN documentation that provided concept coverage of the manually constructed documentation.}
\label{tab:software_docs}
  \addtolength{\tabcolsep}{-4pt}
\begin{tabular}{L{.8cm}L{2.5cm}L{5.1cm}}
\hline
\textbf{Project} & \textbf{Manual}& \textbf{HGEN} \\ \hline
Drono- logy & Each individual UAV that is included in a Mission Plan shall have an ordered list of one or more flight routes assigned to it. & Flight Plan Assignment: The system shall enable users to assign flight plans to specific drones in the fleet by selecting a drone identifier and flight plan to link together. This assignment shall be persisted in the data model. \\ \hline
SAFA & I can select an artifact to view more details. & The system shall visually indicate the selection status of artifact nodes when users click to select them, highlighting the nodes in the graph visualization, to enable users to focus on specific artifacts of interest for further analysis. \\ \hline
JOC & As a user, I want to be able to explore and interact with the world & As a user who wants to explore 3D virtual environments, I want to be able to navigate and view a 3D world from a first person perspective so that I can immerse myself in the virtual environment. \\ \hline
\end{tabular}
\end{table}


==> tables/hypothesis_tests.tex <==
\begin{table}
\centering
\caption{Results of Mann–Whitney U tests. Cases in which the null hypothesis is rejected (i.e., where ($p < 0.05$)) are highlighted and depict cases where one treatment outperformed the other with respect to the quality attribute.}
\label{tab:hypothesis_tests}

\begin{tabular}{p{1cm}ccc}
\hline
\multicolumn{4}{c}{\emph{Human vs. Baseline}} \\
\hline
\textbf{Metric} & \textbf{Human Mean} & \textbf{Baseline Mean} & \textbf{Corrected P-value} \\
\hline
Readability & 3.90 & \colorbox{brightblue}{\bf 4.44} & \textbf{0.002445} \\
Appropriateness & 3.70 & 4.00 & 0.214476 \\
Conciseness & 4.30 & 4.44 & 0.596927 \\
Importance & 4.10 & 4.35 & 0.191984 \\
Usefulness & 3.51 & 3.67 & 0.794294 \\
Helpfulness & 3.82 & 3.88 & 0.990378 \\
\end{tabular}

\begin{tabular}{p{1cm}ccc}
\hline
\multicolumn{4}{c}{\emph{Human vs. HGEN}} \\
\hline
\textbf{Metric} & \textbf{Human Mean} & \textbf{HGEN Mean} & \textbf{Corrected P-value} \\
\hline
Readability & 3.90 & \colorbox{brightblue}{4.38} & \textbf{0.000104} \\
Appropriateness & 3.70 & \colorbox{brightblue}{4.16} & \textbf{0.001493} \\
Conciseness & 4.30 & 4.32 & 0.618787 \\
Importance & 4.10 & 4.33 & 0.095525 \\
Usefulness & 3.51 & \colorbox{brightblue}{4.14} & \textbf{7.09e-06} \\
Helpfulness & 3.82 & \colorbox{brightblue}{4.21} & \textbf{0.002445} \\
\end{tabular}

\begin{tabular}{p{1cm}ccc}
\hline
\multicolumn{4}{c}{\emph{Baseline vs. HGEN}} \\
\hline
\textbf{Metric} & \textbf{Baseline Mean} & \textbf{HGEN Mean} & \textbf{Corrected P-value} \\
\hline
Readability & 4.44 & 4.38 & 0.990378 \\
Appropriateness & 4.00 & 4.16 & 0.462604 \\
Conciseness & 4.44 & 4.32 & 0.990378 \\
Importance & 4.35 & 4.33 & 0.990378 \\
Usefulness & 3.67 & \colorbox{brightblue}{4.14} & \textbf{0.020646} \\
Helpfulness & 3.88 & 4.21 & 0.172422 \\
\hline
\end{tabular}
\vspace{-12pt}
\end{table}


==> tables/pilot_meta_data.tex <==
\begin{table}
    \centering
     \caption{HGEN was used in nine industrial Pilot Projects from multiple domains with the source code layer written in diverse programming languages.}
  
    \label{tab:pilots}
      \addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{|c|l|c|c|c|c|l|c|}
    \hline
    \multirow{2}{*}{\textbf{ID}} &
    \multirow{2}{*}{\textbf{Category}} &
    \multicolumn{3}{c|}{\textbf{Use Case}} &
    \multirow{2}{*}{\textbf{ID}} &
    \multirow{2}{*}{\textbf{Lang.}} & \multirow{2}{*}{\textbf{Input Files}}\\ \cline{3-5} %\cline{8-10}
    && RE. & LG & OB & && \\ \hline
      
    \multirow{2}{*}{C1} & \multirow{3}{*}{Enterprise} & \CIRCLE &\CIRCLE & &P1 & C\# & 1,049  \\ \cline{3-8}
    && \CIRCLE &\CIRCLE && P2 & C++ & 181 \\ \hline
    C2&Automotive*& & && P3 & C++ \textasteriskcentered  & 242 \textasteriskcentered \\    
    \hline
    
    C3 & SAAS & & \CIRCLE && P4 & TS / JS& 264 \\  \hline
    C4 & IT Services & \CIRCLE&&& P5 & Java& 197\\  \hline
    C5 & Aerospace & &\CIRCLE && P6 & C & 345  \\  \hline
    C6 & Education & &&\CIRCLE& P7 & Java & 643\\  \hline
    C7 & Automotive* & &&& P8 & \textasteriskcentered & \textasteriskcentered \\ \hline
    C8 & IT Services & &\CIRCLE&& P9 & Go / TS & 65 \\  \hline
    \multicolumn{8}{c}{*Pilot conducted using Open-Source Systems}\\  \multicolumn{8}{c}{RE=Reverse Engineering, LG=Legacy Documentation, OB=Onboarding}\\
    \multicolumn{8}{c}{JS= Java Script, TS = Type Script}
    \end{tabular}
    \vspace{-12pt}
   
\end{table}

==> tables/projects.tex <==
% Fixed the annoying misalignment problem.
\begin{table}
\centering
\caption{The first study evaluated the quality of manually constructed documentation, HGEN, and a baseline approach. Types and numbers of artifacts are depicted for each project. Open-Source datasets are annotated with an asterisk (*).}
\label{tab:projects}
\begin{tabular}{@{}p{4.5cm}p{3.5cm}@{}}
\toprule
\textbf{Dronology *} \cite{DBLP:journals/corr/abs-1804-02423} \newline 
Dronology is an Open-Source small Unmanned Aerial System (sUAS) written in Java. It provides a platform for controlling and coordinating multiple sUAS to support search-and-rescue, surveillance, and scientific data collection missions.
&
\vspace{-12pt}
\raisebox{-\height}{\raggedright\includesvg[inkscapelatex=false,width=3.5cm]{imgs/tims/dronology-tim-noborders.svg}}  \\ 

\vspace{2pt}\textbf{SAFA} \cite{DBLP:conf/kbse/RodriguezNDC22,DBLP:journals/software/Cleland-HuangAV21}\newline 
SAFA is a software documentation management platform that leverages live traceability to build a knowledge graph and support change impact analysis. Our industry collaborators provided access to client-side source code.
&
\raisebox{-\height}{\centering\includesvg[width=3.5cm]{imgs/tims/safa-tim.svg}}\\

\vspace{2pt}\textbf{Jack of Clubs *}  \newline 
Jack of Clubs is a re-creation of Ace of Spades, a voxel-based first-person shooter game. The creator gave us access to the manually created user stories and epics, and we are releasing them to the public as part of this paper.
&
\raisebox{-\height}{\centering\includesvg[width=3.5cm]{imgs/tims/joc-tim.svg}}\\ 
\bottomrule
\end{tabular}
\vspace{-12pt}
\end{table}

% \begin{table}
% \centering
% \caption{Three projects used for evaluation. The graphs shows the types and numbers of artifacts selected for evaluation for each of the human-made documentation, the baseline-method's documentation, and HGEN's documentation. The two Open-Source datasets are annotated with an asterisk (*).}
% \jch{TODO: convert SVG to pdf and then clip to align properly.}
% \label{tab:projects}
% \begin{tabular}{@{}L{4.5cm}L{3.5cm}@{}}
% \toprule
%  \textbf{Dronology *} \cite{DBLP:journals/corr/abs-1804-02423} \newline Dronology is an Open-Source small Unmanned Aerial System (sUAS) written in Java. It provides a platform for controlling and coordinating multiple sUAS to support search-and-rescue, surveillance, and scientific data collection missions.&\raisebox{-\height}{\includesvg[inkscapelatex=false,width=3.5cm]{imgs/tims/dronology-tim-noborders.svg}}  \\ 
 
% \textbf{SAFA} \cite{DBLP:conf/kbse/RodriguezNDC22,DBLP:journals/software/Cleland-HuangAV21}\newline SAFA is a software documentation management platform that leverages live traceability to build a knowledge graph and support change impact analysis. Our industry collaborators provided access to client-side source code.&\raisebox{-\height}
% { \includesvg[width=3.5cm]{imgs/tims/safa-tim.svg}}\\

% \textbf{Jack of Clubs *}  \newline Jack of Clubs is a re-creation of Ace of Spades, a voxel-based first-person shooter game. The creator gave us access to the manually created user stories and epics, and we are releasing them to the public as part of this paper.&\raisebox{-\height}{\includesvg[width=3.5cm]{imgs/tims/joc-tim.svg}}\\ \bottomrule
% \end{tabular}
% \end{table}


==> tables/quality_metrics.tex <==
\begin{table}[]

  \addtolength{\tabcolsep}{-3pt}
    \centering
    \small


\caption{Evaluation guidelines for assessing documentation quality.}
\label{tab:quality_metrics}
\small
   %\color{MediumBlue} 
\begin{tabular}{|L{1.2cm}|L{1.6cm}|L{5.3cm}|}
\hline
\textbf{Group} & \textbf{Metric} & \textbf{Metric Description} \\ \hline
Language & Readability & How easily a user can understand the information provided. \\ \cline{2-3}

& Appropriate-ness & Language appropriateness with respect to the artifact's technical level. \\
\hline
Content & Conciseness & How brief, yet clear the system is described.\\
\cline{2-3}
& Importance & Considers the importance of the information provided.
\\
\hline
Effective-ness & Usefulness & Considers how useful this documentation is to the project expert. \\
\cline{2-3}
& Helpfulness & Consider how helpful the documentation is for understanding its children. \\
\hline
\end{tabular}
\vspace{-12pt}
\end{table}


==> tables/tracing.tex <==
\begin{table}
\centering
\label{tab:tracing}
\caption{Traceability Accuracy Metrics for Generative Approaches}
\begin{tabular}{llcccc}
\hline
\textbf{Project} & \textbf{Approach} & \textbf{mAP} & \textbf{Precision} & \textbf{Recall} & \textbf{\# Orphans} \\ \hline \hline
\multirow{2}{*}{Dronology} & Baseline & 84.5\% & 47.2\% & 89.5\% & 17 \\
 & HGEN & 94.0\% & 56.3\% & 93.4\% & 0 \\ \hline
\multirow{2}{*}{SAFA} & Baseline & 91.9\% & 49.2\% & 100\% & 28 \\
 & HGEN & 94.5\% & 54.3\% & 98.4\% & 9 \\ \hline
\multirow{2}{*}{JOC} & Baseline & 95.5\% & 67.3\% & 74.5\% & 11 \\
 & HGEN & 96.7\% & 81.4\% & 80.2\% & 1 \\ \hline
\end{tabular}
\end{table}

==> temp.tex <==
 \mdfdefinestyle{MyFrame}{%
    linecolor=gray,
    outerlinewidth=.5pt,
    roundcorner=0pt,
    % innertopmargin=\baselineskip,
    % innerbottommargin=\baselineskip,
    innerrightmargin=6pt,
    innerleftmargin=6pt,
    backgroundcolor=gray!20
}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%%%%%%%%%%%%%% CUSTOM COMMANDS %%%%%%%%%%%%%%
\newcommand{\latinphrase}[1]{\textit{#1}}
\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\newcommand{\smalltt}[1]{{\small\texttt{#1}}}
\newcommand{\citesec}[1]{Section~\ref{sec:#1}}
\newcommand{\citefig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\citealgo}[1]{\textsc{Listing}~\ref{algo:#1}}
\newcommand{\citelisting}[1]{\textsc{Listing}~\ref{lst:#1}}
\newcommand{\citetable}[1]{{Table}~\ref{tab:#1}}
\newcommand{\citedef}[1]{\textsc{Definition}~\ref{def:#1}}

\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash}p{#1}} 


\newcommand{\etal}{\emph{et~al.}\xspace}
\newcommand{\fwname}{\textit{xxx}\xspace}

\newcommand{\MtoH}{\textbf{$[M \rightarrow H]$}\xspace}
\newcommand{\HtoM}{\textbf{$[H \rightarrow M]$}\xspace}

% \newcommand{\jch}[1]{{\textcolor{blue}{#1}}} %blue
% \newcommand{\kd}[1]{{\textcolor{red}{#1}}} %red

% \definecolor{dkgreen}{HTML}{006400}
% \newcommand{\ar}[1]{\textcolor{dkgreen}{#1}} %green
\definecolor{grayhighlight}{rgb}{.65,0.65,0.65}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{LightAmber}{rgb}{0.98,0.89,0.74}
\definecolor{menthol}{rgb}{0.64, 0.98, 0.64}
\newcommand*{\mybox}[2]{\colorbox{#1!30}{\parbox{.98\linewidth}{#2}}}

\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}
\newcommand{\hlt}[1]{{\textcolor{alizarin}{#1}}}%orange
\newcommand{\markphase}{ \CIRCLE}
\hyphenation{autono-mous}
